Benchmarking Approximate Inference Methods for Neural Structured Prediction

Exact structured inference with neural network scoring functions is computationally challenging but several methods have been proposed for approximating inference. One approach is to perform gradient descent with respect to the output structure directly (Belanger and McCallum, 2016). Another approach, proposed recently, is to train a neural network (an "inference network") to perform inference (Tu and Gimpel, 2018). In this paper, we compare these two families of inference methods on three sequence labeling datasets. We choose sequence labeling because it permits us to use exact inference as a benchmark in terms of speed, accuracy, and search error. Across datasets, we demonstrate that inference networks achieve a better speed/accuracy/search error trade-off than gradient descent, while also being faster than exact inference at similar accuracy levels. We find further benefit by combining inference networks and gradient descent, using the former to provide a warm start for the latter.

==> sgd-table-new.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{l|c|c||c|c||c|c|}
\cline{2-7}
& \multicolumn{2}{c||}{Twitter POS Tagging}
& \multicolumn{2}{c||}{NER}
& \multicolumn{2}{c|}{CCG Supertagging}
\\ \cline{2-7} 
& Acc. & Energy   & F1 & Energy  & Acc. & Energy  \\
\hline
\multicolumn{1}{|l|}{gold standard} & 100 & -159.65 &100    & -230.63 &  100 &  -480.07  \\
\hline \hline
\multicolumn{1}{|l|}{\blstmcnncrf/Viterbi} &90.9  & -163.20 & 91.6   & -231.53 & 94.3  & -483.09   \\
\hline \hline
\multicolumn{1}{|l|}{gradient descent, $N = 10$} & 89.2 & -161.69 &81.9 & -227.92 & 65.1 &-412.81  \\
\multicolumn{1}{|l|}{$N = 20$} &90.8  & -163.06 &  89.1  & -231.17 &  74.6 & -414.81   \\
\multicolumn{1}{|l|}{$N = 30$} & 90.8 & -163.02 & 89.6 & -231.30 & 83.0 & -447.64\\
\multicolumn{1}{|l|}{$N = 40$} & 90.7 & -163.03 &  89.8  & -231.34 & 88.6  &-471.52    \\
\multicolumn{1}{|l|}{$N = 50$} & 90.8 & -163.04 &  89.8  & -231.35 &  90.0 &-476.56    \\
\multicolumn{1}{|l|}{$N = 100$} & - & - &  -  & - &  90.1 &-476.98    \\
\multicolumn{1}{|l|}{$N = 500$} & - & - & -  & - &  90.1 &-476.99    \\
\multicolumn{1}{|l|}{$N = 1000$} &- & - &  -  & - &  90.1 &-476.99    \\
\hline \hline
\multicolumn{1}{|l|}{inference network} & 91.3 & -162.07 &  90.8  & -231.19 & 94.2 & -481.32    \\
\multicolumn{1}{|l|}{discretized output from inference network} & 91.3 & -160.87 & 90.8   & -231.34 & 94.2  & -481.95    \\
\hline \hline
%\multicolumn{1}{|l|}{inference network + gradient descent, $N = 1$} &  &  &  &  &  & -    \\
\multicolumn{1}{|l|}{Instance-Tailored Inference Network, $N = 3$} &91.0  &-162.59  &91.3  &-231.32  & 94.3 & -481.91    \\
\multicolumn{1}{|l|}{Instance-Tailored Inference Network, $N = 5$} & 90.9 & -162.81 & 91.2 & -231.37 & 94.3 &  -482.23   \\
\multicolumn{1}{|l|}{Instance-Tailored Inference Network, $N = 10$} & 91.3 & -162.85 & 91.5 & -231.39 & 94.3 & -482.56    \\
\hline \hline
\multicolumn{1}{|l|}{inference network + gradient descent, $N = 3$} &91.4  &-163.06  & 91.4 & -231.42 & 94.4 &-482.62     \\
\multicolumn{1}{|l|}{inference network + gradient descent, $N = 5$} & 91.2 & -163.12  & 91.4 & -231.45 & 94.4 & -482.64    \\
\multicolumn{1}{|l|}{inference network + gradient descent, $N = 10$} &91.2  & -163.15 & 91.5 & -231.46 &  94.4& -482.78    \\
\hline
\end{tabular}
\vspace{-0.2cm}
\caption{Test set results for three tasks of the two families of approximate inference methods, showing performance metrics (accuracy and F1) as well as average energy of the output of each method.\lifu{adding experiment results} 
%Gradient descent inference results are obtained when there are no improvement if increasing number of iterations with the tuning learning rate. \kevin{Not sure I understand this sentence.. how did you tune the learning rate?}. \lifu{changed} \kevin{notable improvement in energy or accuracy?} 
The inference network architectures in the above experiments are: CNN for POS, seq2seq for NER, and BLSTM for CCG.
%\kevin{Oh, why did you use BLSTM for CCG? The earlier \blstmcnncrf results used seq2seq for CCG, right?}\lifu{I get results of seq2seq and BLSTM for CCG before. However, BLSTM got a little higher performance.}
}
\label{table:sgd}
\vspace{-0.3cm}
\end{table*}

==> sgd_test.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lc|c|c||c|c||c|c|}
\cline{3-8}
&& \multicolumn{2}{c||}{Twitter POS Tagging}
& \multicolumn{2}{c||}{NER}
& \multicolumn{2}{c|}{CCG Supertagging}
\\ \cline{3-8} 
& $N$ & Acc. $(\uparrow)$ & Energy $(\downarrow)$   & F1 $(\uparrow)$ & Energy $(\downarrow)$ & Acc. $(\uparrow)$ & Energy  $(\downarrow)$ \\
\hline
\multicolumn{1}{|l}{gold standard} &  & 100 & -159.65 &100    & -230.63 &  100 &  -480.07  \\
\hline \hline
\multicolumn{1}{|l}{\blstmcnncrf/Viterbi} &  & 90.9  & -163.20 & 91.6   & -231.53 & 94.3  & -483.09   \\
\hline \hline
\multicolumn{1}{|l}{} & 10 & 89.2 & -161.69 &81.9 & -227.92 & 65.1 &-412.81  \\
\multicolumn{1}{|l}{} & 20 &90.8  & -163.06 &  89.1  & -231.17 &  74.6 & -414.81   \\
\multicolumn{1}{|l}{} & 30 & 90.8 & -163.02 & 89.6 & -231.30 & 83.0 & -447.64\\
\multicolumn{1}{|l}{\multirow{2}{*}{gradient descent}} & 40 & 90.7 & -163.03 &  89.8  & -231.34 & 88.6  &-471.52    \\
\multicolumn{1}{|l}{} & 50 & 90.8 & -163.04 &  89.8  & -231.35 &  90.0 &-476.56    \\
\multicolumn{1}{|l}{} & 100 & - & - &  -  & - &  90.1 &-476.98    \\
\multicolumn{1}{|l}{} & 500 & - & - & -  & - &  90.1 &-476.99    \\
\multicolumn{1}{|l}{} & 1000 &- & - &  -  & - &  90.1 &-476.99    \\
\hline \hline
\multicolumn{2}{|l|}{$\infnetLarge$} & 91.3 & -162.07 &  90.8  & -231.19 & 94.2 & -481.32    \\
\multicolumn{2}{|l|}{discretized output from $\infnetLarge$} & 91.3 & -160.87 & 90.8   & -231.34 & 94.2  & -481.95    \\
\hline \hline
\multicolumn{1}{|l}{} & 3 &91.0  &-162.59  &91.3  &-231.32  & 94.3 & -481.91    \\
\multicolumn{1}{|l}{instance-tailored $\infnetLarge$} & 5 & 90.9 & -162.81 & 91.2 & -231.37 & 94.3 &  -482.23   \\
\multicolumn{1}{|l}{} & 10 & 91.3 & -162.85 & 91.5 & -231.39 & 94.3 & -482.56    \\
\hline \hline
\multicolumn{1}{|l}{\multirow{2}{*}{$\infnetLarge$ as warm start for}} & 3 &91.4  &-163.06  & 91.4 & -231.42 & 94.4 &-482.62     \\
\multicolumn{1}{|l}{\multirow{2}{*}{gradient descent}} & 5 & 91.2 & -163.12  & 91.4 & -231.45 & 94.4 & -482.64    \\
\multicolumn{1}{|l}{} & 10 &91.2  & -163.15 & 91.5 & -231.46 &  94.4& -482.78    \\
\hline
\end{tabular}
\vspace{-0.1cm}
\caption{Test set results of approximate inference methods for three tasks, showing performance metrics (accuracy and F1) as well as average energy of the output of each method. 
The inference network architectures in the above experiments are: CNN for POS, seq2seq for NER, and BLSTM for CCG. $N$ is the number of epochs for GD inference or instance-tailored fine-tuning. 
}
\label{table:sgd}
\vspace{-0.2cm}
\end{table*}

